Data Augmentation for Deep Graph Learning: A Survey

Graph neural networks, a powerful deep learning tool to model graph-structured data, have demonstrated remarkable performance on numerous graph learning tasks. To address the data noise and data scarcity issues in deep graph learning, the research on graph data augmentation has intensified lately. However, conventional data augmentation methods can hardly handle graph-structured data which is defined in non-Euclidean space with multi-modality. In this survey, we formally formulate the problem of graph data augmentation and further review the representative techniques and their applications in different deep graph learning problems. Specifically, we first propose a taxonomy for graph data augmentation techniques and then provide a structured review by categorizing the related work based on the augmented information modalities. Moreover, we summarize the applications of graph data augmentation in two representative problems in data-centric deep graph learning: (1) reliable graph learning which focuses on enhancing the utility of input graph as well as the model capacity via graph data augmentation; and (2) low-resource graph learning which targets on enlarging the labeled training data scale through graph data augmentation. For each problem, we also provide a hierarchical problem taxonomy and review the existing literature related to graph data augmentation. Finally, we point out promising research directions and the challenges in future research.

==> IEEEtran/ReadingList.tex <==
\section{Reading List} \heuristic, \automating, \feature, \structure, \llabel
\subsection{Adversarial Training on Graphs}
\begin{itemize}
    \item Batch virtual adversarial training for graph convolutional networks~\cite{deng2019batch}: Consider perturb multiple nodes without overlap (hence avoid sub-optimal perturbation due to the inter-connections). \automating, \feature
    \item Graph adversarial training: Dynamically regularizing based on graph structure~\cite{feng2019graph}: Perturbation is on the attribute of nodes only. Similar idea as AT and VAT. \automating, \feature
    \item Virtual adversarial training on graph convolutional networks in node classification~\cite{sun2019virtual}: Almost the same as `Graph adversarial training: Dynamically regularizing based on graph structure'. \automating, \feature
    
    \item FLAG: Adversarial Data Augmentation for Graph Neural Networks~\cite{kong2020flag}: Basically it is the same as adversarial training, but it does the perturbation and training simultaneously (without finish the training and then computing the hyper-gradient of data samples). \automating, \feature
    
    \item Latent Adversarial Training of Graph Convolution Networks~\cite{jin2019latent}: Add a adversarial training-based regularization term into the objective function which is based on the perturbation of \emph{`intermediate' embedding} but not the input features/topology. \automating, \feature. Augment on the embedding space.
\end{itemize}

\subsection{Contrastive Learning on Graphs}
\begin{itemize}
    \item Deep Graph Infomax~\cite{velickovic2019deep}: Positive samples are the embeddings from GNNs and negative samples are generated by shuffling the rows of feature matrix. \heuristic, \feature
    \item Deep Graph Contrastive Representation Learning~\cite{zhu2020deep}: Generate a corruption graph (view) by randomly dropping edges/features. \heuristic, \feature, \structure
    \item Graph contrastive learning with adaptive augmentation~\cite{zhu2021graph}: Based on `Deep Graph Contrastive Representation Learning', reweighting the corruption probability based on the centrality measure. \heuristic, \feature, \structure
    % \item {\color{red}Graph Representation Learning via Graphical Mutual Information Maximization}~\cite{peng2020graph}
    \item Contrastive Multi-View Representation Learning on Graphs~\cite{hassani2020contrastive}: Focus on augment the structure of graph. Consider adjacency and diffusion matrices as two congruent structural views. \heuristic, \structure 
    
    \item Graph Contrastive Learning with Augmentations~\cite{you2020graph}: Construct contrastive samples using given policies. \heuristic, \feature, \structure
    
    \item Adversarial Graph Augmentation to Improve Graph Contrastive Learning~\cite{suresh2021adversarial}: The encoder aims to maximize the mutual information between the augmented components but the augmenter are optimized in the opposing direction to form the two-player game. The augmenter is parameterized by another GNN with Gumbel-Max reparametrization trick. \automating, \structure
    
    \item Graph contrastive learning automated~\cite{DBLP:conf/icml/YouCSW21}: it follows the work `Graph Contrastive Learning with Augmentations' with learnable probability to select the combination of two augmentation strategies. The scale of search space (for augmentation) is the square of the number of augmentation strategies. \automating, \feature, \structure
    
    \item AutoGCL: Automated Graph Contrastive Learning via Learnable View Generators~\cite{yin2021autogcl} It adopts two strategies: node dropping and attribute masking, whose node-wise decision is made from learnt node feature and after a Gumbel-softmax. \automating, \feature, \structure
\end{itemize}

\subsection{Imbalanced Setting}
\begin{itemize}
    \item Multi-class imbalanced graph convolutional network learning~\cite{shi2020multi}: Generate label-dependent fake nodes (by GAN) and distinguish it from the real nodes to force the GNNs to learn label-specific representation. 
    \automating, \feature, \structure, \llabel
    \item GraphSMOTE: Imbalanced Node Classification on Graphs with Graph Neural Networks~\cite{zhao2021graphsmote}: GNNs get embeddings; SMOTE (KNN-based) to interpolate the embedding space, and use edge predictor to link the generated nodes with existing nodes. 
    \heuristic, \feature, \structure, \llabel
    \item ImGAGN: Imbalanced Network Embedding via Generative Adversarial Graph Networks~\cite{qu2021imgagn}: Generate fake minority nodes and using GAN to discriminate if it is the real minority node. 
    \automating, \feature, \structure
    
    \item GraphMixup: Improving Class-Imbalanced Node Classification on Graphs by Self-supervised Context Prediction~\cite{wu2021graphmixup}. \heuristic, \feature, \structure, \llabel

\end{itemize}

\subsection{Learning on Disassortative/Heterophilic Graphs}

\begin{itemize}
    \item Breaking the limit of graph neural networks by improving the assortativity of graphs with local mixing patterns~\cite{DBLP:conf/kdd/SureshBNLM21}: Augment various types of edges based on the structural similarity to improve the assortativity of given graphs. \heuristic, \structure.
    
    \item GCN-SL: Graph Convolutional Network with Structure Learning for Disassortative Graphs~\cite{jiang2021gcn}: Modify the given adjacency matrix based on transformed node feature to construct more assortative connections. \heuristic, \structure
    
    \item Geom-gcn: Geometric graph convolutional networks~\cite{pei2019geom}: Enriching the computation graph through the geometric relationship in the learned latent space. \automating, \structure
    
    \item Sparse graph attention networks~\cite{ye2021sparse}. \automating, \structure
    
    \item Adaptive filter works.
    
    
\end{itemize}

\subsection{Others}
\begin{itemize}
    \item Data augmentation for graph neural networks~\cite{zhao2021data}: Decompose and reconstruct the graphs based on GNN and using the reconstruction matrix to add/delete edges. \automating, \structure
    
    
    \item Deeper Insights into Graph Convolutional Networks for Semi-Supervised Learning~\cite{li2018deeper}: Expand the label sets via pair walk / self-training. \heuristic, \automating, \llabel
    
    
    \item GraphMix- Regularized Training of Graph Neural Networks for Semi-Supervised Learning~\cite{verma2019graphmix}: Cotraining FCN and GNN but with shared parameters. Specifically adopting mixup in the training of FCN. \automating, \feature, \llabel
    
    \item Semi-supervised learning on graphs with generative adversarial nets~\cite{ding2018semi}: Design the loss of G and D to push the generating samples in the middle of density gap. \automating, \feature. Augment on the embedding space.
    
    \item Node Augmentation Methods for Graph Neural Network based Object Classification~\cite{xue2021node}: Add new nodes into the graph, and then mixup the corresponding features, topology (by continuous or discrete methods), and labels. \heuristic, \feature, \structure, \llabel
    
    \item Labeling Trick: A Theory of Using Graph Neural Networks for Multi-Node Representation Learning~\cite{zhang2021labeling}: Labelling the nodes with some extra dimension when doing the prediction to distinguish them with the non-target nodes. \heuristic, \feature
    
    \item Neural Message Passing for Quantum Chemistry~\cite{gilmer2017neural}: Add virtual edges between unconnected nodes and add a virtual node connecting to all the existing nodes to augment the given graph. Structure-level augmentation.
    \heuristic, \structure
    
    \item Learning Graph-Level Representation for Drug Discovery~\cite{li2017learning}: Introducing a super node to learn the graph-level representation where all the original nodes link to the super node through directed edges. \heuristic, \structure
    
    \item Graph Warp Module: an Auxiliary Module for Boosting the Power of Graph Neural Networks in Molecular Graph Analysis~\cite{ishiguro2019graph}: Apply a supernode to improve the information propagation of the whole graph for the molecular analysis task. \heuristic, \structure
    
    \item Graph Classification via Deep Learning with Virtual Nodes~\cite{pham2017graph}: Add a virtual node connecting to all the existing nodes with bidirectional links. The node representation of the virtual node denotes the representation of the graph. Similar to `Learning Graph-Level Representation for Drug Discovery'. \heuristic, \structure
    
    \item Local Augmentation for Graph Neural Networks~\cite{liu2021local}: Generate multiple sets of feature matrices as the augmentation, which is based on generative models. Feature generation. \automating, \feature
    
    \item Pre-train and Learn: Preserve Global Information for Graph Neural Networks~\cite{zhu2019pre}: Based on deepwalk-based methods to generate augmented node features and combine the output of several GNNs (fed with different features) to output the final prediction. Feature generation. \automating, \feature
    
    \item NodeAug: Semi-Supervised Node Classification with Data Augmentation~\cite{wang2020nodeaug}: Replace attributes, add/delete edges based on some heuristics, and then keep the output consistency before and after the augmentation. Feature calibration, node addition \& removing. \heuristic, \feature, \structure
    
    \item Identity-aware Graph Neural Networks~\cite{you2021identity}: A fast algorithm proposed by the authors is using cycle counts as augmented node features. Feature generation. \heuristic, \feature
    
    \item Adaptive Data Augmentation on Temporal Graphs~\cite{wang2021adaptive}: Augment temporal graphs by \textbf{perturbing both the time and edge} adaptively by considering the influence of `time distance' and `topology distance'. Edge addition/ removing and more (time perturbation). \heuristic, \structure
    
    \item Robust Graph Representation Learning via Neural Sparsification
\end{itemize}

\subsection{Tutorials \& Lectures}
\begin{itemize}
    \item 
\end{itemize}
